Range (R\'enyi) Entropy Queries and Partitioning

Data partitioning that maximizes/minimizes the Shannon entropy, or more generally the R\'enyi entropy is a crucial subroutine in data compression, columnar storage, and cardinality estimation algorithms. These partition algorithms can be accelerated if we have a data structure to compute the entropy in different subsets of data when the algorithm needs to decide what block to construct. Such a data structure will also be useful for data analysts exploring different subsets of data to identify areas of interest. While it is generally known how to compute the Shannon or the R\'enyi entropy of a discrete distribution in the offline or streaming setting efficiently, we focus on the query setting where we aim to efficiently derive the entropy among a subset of data that satisfy some linear predicates. We solve this problem in a typical setting when we deal with real data, where data items are geometric points and each requested area is a query (hyper)rectangle. More specifically, we consider a set $P$ of $n$ weighted and colored points in $\mathbb{R}^d$, where $d$ is a constant. For the range S-entropy (resp. R-entropy) query problem, the goal is to construct a low space data structure, such that given a query (hyper)rectangle $R$, it computes the Shannon (resp. R\'enyi) entropy based on the colors and the weights of the points in $P\cap R$, in sublinear time. We show conditional lower bounds proving that we cannot hope for data structures with near-linear space and near-constant query time for both the range S-entropy and R-entropy query problems. Then, we propose exact data structures for $d=1$ and $d>1$ with $o(n^{2d})$ space and $o(n)$ query time for both problems. Finally, we propose near linear space data structures for returning either an additive or a multiplicative approximation of the Shannon (resp. R\'enyi) entropy in $P\cap R$.

==> coverletter.tex <==
\thispagestyle{empty} % no page number
\vspace{-2em}
\begin{center}
{\Large Cover Letter}
\end{center}
%\vspace*{\fill}

We would like to thank the authors for their thoughtful and useful comments.
We made all required changes and addressed the reviewers’ comments. We have highlighted all changes in the revised manuscript in {\color{blue}blue}. In summary, we made the following main changes in this revision:
\begin{itemize}
    \item We improved the motivation by adding citations to the previous examples and including a new example motivating the \renyi entropy. (R1)
    \item We revised the final statements of some of our lower bounds. (R1)
    \item We elaborated on the connection between our problem and colored range searching, and we compared it with additional related work. (R2, R3)
    \item We provided more details on the range sampling data structures. (R2)
    \item We now present the exact data structures using \renyi entropy and straightforwardly extend to Shannon entropy. (R2)
    \ifshowcomments
    \item We added a new space-query tradeoff lower bound for $d=1$. (R2)
    \fi
\end{itemize}


In the rest of the cover letter, we respond to all comments individually and
explain the set of actions we took to resolve them.

\paragraph{Reviewer 1}

R1.1) page 2:  The instances where entropy shows up in Compression,
Probability, and TCS should specify if these are for Shannon or Renyi
entropy.  In particular, Renyi entropy is less well known, so please
make sure to include a clear motivating example where it is needed.

\new{Ans: For each example, we now specify whether it is related to Shannon or \renyi entropy and include supporting citations. Additionally, we have incorporated a new example illustrating \renyi entropy.}

\vspace{1.5em}

R1.2) page 2,3:  Please suggest what are common values of alpha to use for
Renyi Entropy (e.g., in Diversity index).  Is it normally alpha=2, or
maybe much larger?

\new{Ans: We added the most common values of $\alpha$ which are $\alpha \rightarrow 1, \alpha=2$, and $\alpha \rightarrow \infty$.}

\vspace{1.5em}

R1.3) page 4:
   "constructing near linear data structures" $->$ "constructing near
linear size data structures"
   "these are an efficient" $->$ "these are efficient"

\new{Ans: We fixed the typos.}

\vspace{1.5em}

R1.4) page 9,10:
   Please add a bit more detail (perhaps in an appendix) for two
critical aspects of the entropy update equations:
   - explain the weighted versions
   - a few more steps in deriving the Renyi update step (or provide a
citation)

\new{Ans: For the weight version, we only need to replace $|P_1|, |P_2|, |P_3|$ with $w(P_1), w(P_2), w(P_3)$, respectively. We also included the proofs of the formulas for updating the \renyi entropy in Appendix A.}

\vspace{1.5em}

R1.5) page 14+:  The conditional lower bound theorems are stated as the
Contrapositive of what I would except.  For instance for Theorem 3.2 I
suggest a statement like:

===
If the set intersection problem requires $\Omega((n/Q(n))^2)$ space to
solve on n points with query time $Q(n)$, then range entropy queries for n
points in $R^d$, for constant d, require $\tilde{\Omega}((n/Q(n/2))^2)$ space to
solve in $Q(n)$ query time.
===

Otherwise a rider must take this additional contrapositive step to
understand the hardness of the main topic of this paper, as opposed to
suggesting a reduction.
This is true for other lower bound statements as well.  E.g., it would
be useful on page 16,17 for Thm 3.7, 3.8 to state something like:
   If Matrix Multiplication is hard, then range-entropy requires large
pre-processing.

\new{
Ans:
Thank you for the comment. We have added Corollary~\ref{cor:prep-tradeoff} following Theorem~\ref{thm:Renlb} (formerly Theorem 3.2), presenting the result as the reviewer suggested. We retained Theorem~\ref{thm:Renlb} because it is more general and can potentially be applied to other conjectures related to the set intersection problem.

Multiple lower bounds exist for the subsequent result on preprocessing time. We revised Theorem~\ref{theorem:r-matrix} according to the reviewer’s suggestion. However, we chose not to present a single explicit lower bound, since several are known (both combinatorial and non-combinatorial) for the multiplication of two Boolean tables, as noted in the Interpretation paragraph. If the reviewer prefers, we can instead present one specific lower bound, such as the combinatorial result from [Sat94, Lee02], and revise Theorem~\ref{theorem:r-matrix} accordingly.}

\vspace{1.5em}

R1.6) page 39,40:  Start of Section 7
   "as this is mostly the case" and "Except of being a ..." could use
some word smithing.

\new{Ans: We fixed it.}

\vspace{1.5em}

R1.7) This section says it will "skip the $\log(n)$ factors"   Its better to
write this with a $\tilde{O}$ notation then, explaining that it omits $\log(n)$
Dependence.

\new{Ans: We introduced and used the $\tilde{O}$ notation.}

\vspace{1.5em}

\paragraph{Reviewer 2}

R2.1) In my opinion, colored range searching is very related here and thus it should be discussed earlier and with more depth.

\new{Ans: We added a short paragraph after defining the range S-entropy and R-entropy queries, and we expanded the discussion of colored range searching in the Related Work.}

\vspace{1.5em}

R2.2) Also, in terms of citations, the paper cites DBVKOS08 which is a standard graduate textbook on computational geometry. This could be fine but in my opinion, it is better to cite papers that originate the techniques/data structures. Also cite the survey by Aggarwal on range searching.

\new{Ans: We added the correct citations. We also kept DBVKOS08 because it clearly explains range trees in detail, especially for non-expert readers.}

\vspace{1.5em}

R2.3) Page 9: I buy that we can assume all weights are equal to one but I don't buy that this is "verbatim". For example, if the weights are real numbers, then reservoir sampling is required as well as an assumption that we can generate a random real number between 0 and 1. In particular, the method mentioned in AP19 should be used. Also, in this case, fractional cascading cannot be used, as far as I can see. The paper in general is a bit sloppy in discussing the range sampling data structures. 

\new{Ans: We have added more details about the range tree for sampling queries (Section~\ref{sec:prelim}) and the range tree for sampling queries excluding one color (Subsection~\ref{subsec:ApproxMult}). We also added a paragraph to each explaining how they naturally extend to weighted points.  
In Section~\ref{sec:prelim}, we further provide definitions of the update operations for both Shannon and \renyi entropy in the context of weighted point sets, which clarifies why all of our data structures naturally extend to the weighted setting. In particular, instead of using update operations and uniform sampling for unweighted points, we now use their weighted counterparts.

As noted in Section~\ref{sec:prelim}, although fractional cascading could be applied, we omitted it for simplicity. One reason is that our goal is to present data structures that generalize naturally to the weighted case. Accordingly, all stated query-time complexities are given without fractional cascading. The asymptotic complexities (preprocessing, space, query, and update times) remain the same for both weighted and unweighted settings.

Furthermore, while more efficient data structures for range weighted sampling in $\mathbb{R}^d$ exist, we are not aware if we can trivially extended them to exclude a color while maintaining their efficient query time. Moreover, they do not improve the asymptotic running time of our query procedures. For example, the data structure of [Mar20] can obtain $t$ samples in $O(\log^d n + t \log n)$ time, whereas our data structure returns $t$ samples in $O(t \log^d n)$ time. In all instances where sampling is required in our data structures, each sample query is paired with a counting or weighted-sum query (in the weighted case). We are not aware of any method that supports $t$ such queries faster than $O(t \log^d n)$ time.  
In any case, throughout the paper, we do not aim to optimize the $\log n$ factors. Instead, our focus is on designing near-linear space (approximate) data structures for: i) range S-entropy queries with $O(\polylog n)$ query time, and ii) range R-entropy queries with $O(n^{1-1/\alpha} \polylog n)$ query time, excluding the dependency on the error parameters $\eps, \Delta$.

%Furthermore, while AP19 could be used for weighted sampling, it does not improve the overall asymptotic query time. Our data structures for weighted sampling take $O(t \cdot \log^d n)$ to sample $t$ samples. Optimized data structures like in AP19 can do sampling in $O()$

%Moreover, we are not aware if it is trivial to extend AP19 to cases excluding the points of a color, as the data structure we need in Section 5.2.

Finally, we removed the word “verbatim” and now simply state that all our data structures extend straightforwardly to the weighted case. 
}

\vspace{1.5em}

R2.4) Page 16: Why doesn't this reduction apply to the set intersection queries? If so, you get a space hardness result for the 1D version of the problem as well. This needs to be discussed in my opinion.


\new{
\ifshowcomments
Thank you for the great observation. Indeed, we can get a space-query tradeoff lower bound for $d=1$. We added more details in the end of Subsection~\ref{subsec:space-tradeoff} and state the result in Theorem~\ref{thm:lbd1}.
\else
Ans:
We tried to apply the same idea to set intersection queries, but it is not trivial to get a meaningful result.
%Indeed, the same idea can be applied to set intersection queries. However, the guarantee achieved by this reduction is not meaningful, as the same guarantee can be obtained trivially without using the reduction. 
Assume we are given a set system $S = \{S_1, \cdots, S_g\}$ over a universe $U$ such that $\sum_{i \in [g]}|S_i| = n$. To apply the reduction, the goal is to first construct a range entropy data structure and then answer set intersection queries over $S$ using this data structure. Following the same approach as on Page 16, for each set $S_i \in S$, we first need to construct a set of $|U|$ points, denoted by $A_i$. We then color the last $|S_i|$ points in $A_i$ with colors from the set $S_i$, and the first $|U| - |S_i|$ points with colors from $U \setminus S_i$ for all $i \in [g]$. We perform a similar construction to obtain the sets $B_i$.
By this construction, we have $\sum_{i \in [g]}|A_i| +  \sum_{i \in [g]}|B_i| = 2g|U|$.
Unfortunately, in the general case, we are not aware of any lower bound for the set intersection problem that involves $O(g\cdot |U|)$ space.
However, if $|U|\geq g$, then this reduction leads to a trivial result, since if we allow $O(g^2)$ space for the original set intersection problem, we can simply precompute and store all pairwise intersections (i.e., for each pair of sets, store whether they intersect), enabling $O(1)$ query time.

%Thus, the reduction itself requires $O(n^2)$ space just to represent the input in the format needed for the range entropy problem. This makes the reduction useless, since if we are allowed $O(n^2)$ space for the original set intersection problem, we can simply precompute and store all pairwise intersections (i.e., for each pair of sets, store whether they intersect), enabling $O(1)$ query time. Therefore, reducing set intersection to range entropy in this way offers no advantage, and hence no interesting lower bound can be obtained.

Overall, intuitively, the reason matrix multiplication is amenable to this kind of reduction is that the best known algorithms for multiplying two $h \times h$ matrices require strictly more than $O(h^2)$ time (specifically, $O(h^{\omega})$ for $\omega > 2$). On the other hand, the set intersection problem, having $h$ sets, can be solved using $O(h^2)$ space trivially.
\fi
}


\vspace{1.5em}

R2.5) Page 21: rectangle containment can be solved with 2d dominance queries but it either needs a reference or some short explanation as it is not entirely trivial. 

\new{Ans: We added a citation.}

\vspace{1.5em}

R2.6) Proof of Lemma 5.3 is a bit too hand-wavy. Just use an inequality to demonstrate that because the following is not a mathematical argument: "We have the minimum value of $H(D)$, when $D$ is concentrated over one value. Since there is no index $j$ with $D(xi_j ) > 2/3$, in the worst case we assume there is index j with $D(xi_j ) = 2/3$". Shouldn't you be able to use Lemma 5.6 here or some variants of its proof?

\new{Ans: Indeed, our original argument was too informal. We wrote it this way because the argument is known, but we had forgotten to include the citation [CCM07] (it was cited earlier in the description of the data structure, but not directly in the proof of this lemma). Instead of re-writing the full proof, we now clearly cite [CCM07] and argue that, in our setting, if for every color the fraction of points of that color in a range $R$ is at most $2/3$, then
$H(P \cap R) > 0.9$.
}

\vspace{1.5em}

R2.7) The extension of exact data structures to Renyi entropy is very straightforward and as far as I can see, requires no new ideas, just plugging in formulas for updating Renyi entropy. Why not just remove the original description and just change it to Renyi entropy? In general, there is a lot of repetition in the paper where same techniques are used over and over again between the Renyi and Shannon entropy models. This makes the paper needlessly long and makes for a tedious read. Just combine all the results for Renyi and Shannon entropy in one description since setting $\alpha=1$ gives the result for Shannon entropy anyways. I guess the only exception is the approximate stuff so maybe that can be kept separate. 

\new{Ans: We completely agree that extending the exact data structures to \renyi entropy is straightforward. We have revised the manuscript accordingly and now describe all exact data structures using \renyi entropy. At the end of each exact data structure ($d=1$ and $d\geq 2$), we state that all results can be extended to Shannon entropy by applying the corresponding update functions provided in Section~\ref{sec:prelim}.
Consequently, for $d = 1$ we now present a single theorem covering both Shannon and \renyi entropy, and for $d > 1$ we likewise present one theorem covering both. We do not claim that the results extend to Shannon entropy simply by setting $\alpha = 1$, since \renyi entropy is not defined at $\alpha = 1$ (although Shannon entropy is equal to the limit of \renyi entropy as $\alpha \to 1$). This is why in  Section~\ref{sec:prelim} we provide separate update functions for Shannon and \renyi entropy. Nevertheless, the results for \renyi entropy directly extend to the Shannon entropy.
}

\vspace{1.5em}

R2.8) Section 5.3: Should that be "query interval R"? Also same for the statement of Theorem 5.11. In general, use of the word "hyper-rectangle" in dimensions, 1 or 2 is confusing and should be avoided.

\new{Ans: Thank you for careful reading. We fixed it in Theorem 5.11 and Theorem 6.5.}

\vspace{1.5em}

R2.9) The definition of I is unclear.  The text says it is the set of all the intervals but that would be $n^2$ intervals. This part should a bit better explained. 

\new{Ans: The set $I$ is defined as the set of all intervals having endpoints the points from set $B$. The size of $B$ is $n^{1-t}$, so $|I|=O(n^{2(1-t)})$. We re-wrote this part.}

\vspace{1.5em}

R2.10) Also, finding the maximal $I_{i,j}$ that is contained in the query interval does not need interval tree it only needs two predecessor queries. 

\new{Ans: Indeed, we changed it.}

\vspace{1.5em}

R2.11) page 25: "In other words, in each node ..." there is an extra parenthesis in the definition. Also this definition is not very clear to me, maybe there is a typo here.

\new{Ans: We re-wrote this part.}

\vspace{1.5em}

\paragraph{Reviewer 3}

R3.1) Since the paper deals with weighted colored ranges searching, it might be worth citing some of these computational geometry papers.
Survey paper: Prosenjit Gupta, Ravi Janardan, Saladi Rahul, Michiel Smid. Computational Geometry: Generalized (or Colored) Intersection Searching.
Handbook of Data Structures and Applications, Sartaj Sahni and Dinesh Mehta eds., CRC Press, 2nd Edition.
Papers which have dealt with weighted colored range searching:
Further Results on Colored Range Searching. Timothy M. Chan, Qizheng He, Yakov Nekrich. SoCG 2020.
Data Structures for Range Aggregation by Categories. Saladi Rahul, Prosenjit Gupta, K. S. Rajan. CCCG 2009.
Range Aggregate Structures for Colored Geometric Objects. Saladi Rahul, Haritha Bellam, Prosenjit Gupta, K.S.Rajan. CCCG 2010.

\new{Ans: We would like to thank the reviewer for the suggested citations. We added a short paragraph after defining the range S-entropy and R-entropy queries, and we expanded the discussion of colored range searching in the Related Work including all the suggested citations.}







\newpage
\setcounter{page}{1}

==> oldMultApprox.tex <==
\stavros{Below is the old version-----------}
\mparagraph{Query procedure}
Given a query rectangle $R$, we run a query on $\mathcal{T}$ and we get a set of $k=O(\log^d n)$ canonical nodes $V=\{v_1,\ldots, v_k\}$ whose corresponding rectangles partition $R$. We compute $E=\sum_{i=1}^k |u(P_{v_i})|$.
Then, we run another counting query in $\mathcal{T}$ to get $N=|P\cap R|$.

If $E=O(\sqrt{N}\log^{d/2}n)$ then we run a range color query on $\mathcal{T}$. In particular, we get a set of $O(\log^{d} n)$ canonical subsets containing all colors in $u(P\cap R)$. For each color $u_i\in u(P\cap R)$, we run a query in $\mathcal{T}_i$ finding $N_i$ the number of points with color $u_i$ in $P\cap R$. In the end, we return $h=\sum_{u_i\in u(P\cap R)}\frac{N_i}{N}\log \frac{N}{N_i}$.

Next, if $E=\Omega(\sqrt{N}\log^{d/2}n)$, unfortunately, it is expensive to compute the entropy visiting all colors in $u(P\cap R)$. Instead, we use the algorithm in~\cite{guha2006streaming}.
In particular, we set $H'=\Omega\left(\frac{1}{\sqrt{N}\log^{d/2}n}\right)$ and we
run $O\left(\frac{\log^2 n}{\eps^2\cdot H'}\right)$ oracle queries $\textsf{SAMP}_D$ or $\textsf{EVAL}_D$, as we did in the additive approximation.
In the end we return the estimate $h$.

\mparagraph{Correctness}
We prove that the query procedure returns a value $h$ such that $\frac{1}{1+\eps}H(P\cap R)\leq h\leq (1+\eps)H(P\cap R)$.
First, we argue that $E$ is a good approximation of the number of colors in $P\cap R$. In particular,
\begin{equation}
\label{eq:color-approx}
    |u(P\cap R)|\leq E\leq c\cdot |u(P\cap R)|\cdot \log^d n,
\end{equation}
for a constant $c$.
Recall that $E=\sum_{i=1}^k |u(P_{v_i})|$. We have $\bigcup_i u(P_{v_i})=u(P\cap R)$, so we also have $E\geq |u(P\cap R)|$. Furthermore, each color in $u(P\cap R)$ might exist in all $O(\log^d n)$ $\mathcal{T}$'s canonical nodes $v_i$ that partition $P\cap R$. Hence the result in Equation~\ref{eq:color-approx} follows.

In the first case, since $E=O(\sqrt{N}\log^{d/2} n)$, from Equation~\ref{eq:color-approx} we have that $|u(P\cap R)|=O(\sqrt{N}\log^{d/2} n)$. For each color $u_i$ in $u(P\cap R)$, we compute $N_i$ so the value $h$ we return has the true entropy of $P\cap R$, i.e., $h=H(P\cap R)$.


In the second case, we show that $H'=\Omega\left(\frac{1}{\sqrt{N}\log^{d/2}n}\right)$ is a correct lower bound of $H(P\cap R)$. Using Equation~\ref{eq:color-approx} we have $|u(P\cap R)|\geq \frac{E}{c\cdot \log^d n}=\Omega\left(\frac{\sqrt{N}}{\log^{d/2}n}\right)$. As we pointed out in the previous Subsection, we have a distribution $D$ with $|u(P\cap R)|$ items. We get the minimum entropy when the distribution is far from being uniform. Hence, in our setting, the minimum entropy is encountered when we have $|u(P\cap R)|-1$ colors having exactly one point, and one color having $|P\cap R|-|u(P\cap R)|+1$ points.
We prove it formally in Appendix~\ref{Appndx:minEntropy}.
The minimum entropy is $\sum_{i=1}^{|u(P')|-1}\left(\frac{1}{|P'|}\log|P'|\right)+\frac{|P'|-|u(P')|+1}{|P'|}\log\frac{|P'|}{|P'|-|u(P')|+1}\geq \frac{|u(P')|-1}{N}=\Omega\left(\frac{\sqrt{N}}{N\log^{d/2} n}\right)=\Omega\left(\frac{1}{\sqrt{N}\log^{d/2}n}\right)$. Using this lower bound for $H(P\cap R)$ in~\cite{guha2006streaming}, we get a value $h$ such that $\frac{1}{1+\eps}H(P\cap R)\leq h\leq (1+\eps)H(P\cap R)$.


\mparagraph{Analysis}
In order to compute $E$ and $N$ we need $O(\log^{d} n)$ time in total since we run range queries on $\mathcal{T}$.
In the first case, we note that we need $O(E\cdot\log^d n)=O(\sqrt{N}\log^{3d/2}n)$ time to find $u(P\cap R)$ (as we showed in the correctness proof, $E$ is a good approximation of $|u(P\cap R)|$). This is because $|u(P\cap R)|=O(\sqrt{N}\log^{d/2}n)$ and each color might exist in $O(\log^d n)$ canonical nodes of $\mathcal{T}$. Then for each color $u_i\in u(P\cap R)$ we spend $O(\log^{d-1} n)$ time to find $N_i$. Overall, the first case takes $O(\sqrt{N}\log^{3d/2}n)$ time.
In the second case, each $\textsf{SAMP}_D$ or $\textsf{EVAL}_D$ query takes $O(\log^{d} n)$ time and we run $O\left(\frac{\log^2 n}{\eps^2\cdot H'}\right)$ queries, so in total we have $O\left(\frac{1}{\eps^2}\sqrt{n}\log^{(3d+1)/2} n\right)$ query time.
%We have $N=O(n)$ so the total query time is $O\left(\frac{1}{\eps^2}\sqrt{n}\log^{(3d+1)/2} n\right)$.


\begin{theorem}
\label{thm:mult-approx-old}
Let $P$ be a set of $n$ points in $\Re^d$, where each point is associated with a color, and let $\eps\in(0,1)$ be a parameter. A data structure of $O(n\log^{d}n)$ size can be computed in $O(n\log^{d} n)$ time, such that given a query hyper-rectangle $R$, a value $h$ can be computed in $O\!\!\left(\frac{1}{\eps^2}\sqrt{n}\log^{\frac{3d+1}{2}} n\!\!\right)$ time, such that $\frac{1}{1+\eps}H(P\cap R)\!\leq\!\! h\!\!\leq\! (1+\eps)H(P\!\cap \!R)$, with high probability.
\end{theorem}
